GrappaRE -- A Tool for Efficient Graph Recognition Based on Finite Automata and Regular Expressions

A recent paper by Drewes, Hoffmann, and Minas (GCM 2023 proceedings) has shown that certain graph languages can be defined and efficiently recognized by finite automata when strings over typed symbols are interpreted as graphs. This approach has been implemented in the tool GrappaRE, which is described in this paper. GrappaRE allows for the convenient specification of graph languages through regular expressions, converts each of them into a minimized deterministic finite automaton, and checks whether it can recognize graphs without the need for backtracking. Measurements confirm that recognition runs in linear time.

==> eptcsdata.tex <==
\providecommand{\firstpage}{55}
\providecommand{\publicationstatus}{J. Endrullis, D. Grzelak, T. Heindel and J. Kosiol (Eds):\\ GCM 2023 and GCM 2024\\
EPTCS 417, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.417.4}{10.4204/EPTCS.417.4}}
\pdfoutput=1
\usepackage{ifthen}
\providecommand{\eptcs}{{\sl Electronic Proceedings in Theoretical Computer Science}}
\providecommand{\opa}{, Open Publishing Association}
\providecommand{\finishreference}[6]{#1 #2#3, pp. #4--#5, \doi{10.4204/EPTCS.#2.#6}}
\providecommand{\thisvolume}[2][\eptcs]{%
 \ifthenelse{\equal{#2}{4420}}{\finishreference{#1}{417}{\opa}{134}{156}{8}}{%
 this volume of #1\opa}}

